Hyperon signatures in the PANDA experiment at FAIR

We present a detailed simulation study of the signatures from the sequential decays of the triple-strange pbar p -> {\Omega}+{\Omega}- -> K+{\Lambda}barK- {\Lambda} -> K+pbar{\pi}+K-p{\pi}- process in the PANDA central tracking system with focus on hit patterns and precise time measurement. We present a systematic approach for studying physics channels at the detector level and develop input criteria for tracking algorithms and trigger lines. Finally, we study the beam momentum dependence on the reconstruction efficiency for the PANDA detector.

==> Omega_detector_signatures_submitted/nima_authors.tex <==
%
% PANDA Collaboration  - authorlist - automatically generated by PANDA website
% 30-03-2023 18:06:21
%
\author[1]{Viktor Abazov}
\author[2]{Victor Abramov}
\author[3,4]{Patrick Achenbach}
\author[5]{Orestis Afedulidis}
\author[5]{Lennart Ahrens}
\author[6]{Adeel Akram}
\author[7,8]{Mohammad Al-Turany}
\author[5]{Malte Albrecht}
\author[1]{Gennady Alexeev}
\author[4]{Ahmed Ali}
\author[9]{Anna Alicke}
\author[10]{Claude Amsler}
\author[11]{Evgeny Antokhin}
\author[12]{Gandharva Appagere}
\author[13]{Ingo Augustin}
\author[14,15]{Kazem Azizi}
\author[16]{Pavel Balanutsa}
\author[17]{Alexander Balashoff}
\author[11]{Alexander Yu. Barnyakov}
\author[18]{Gianni Barucca}
\author[7]{Anastasios Belias}
\author[11]{Konstantin Beloborodov}
\author[19]{Roman Bergert}
\author[20]{Andrea Bianconi}
\author[4]{Sebastian Bleser}
\author[21]{Alexander E. Blinov}
\author[11]{Vladimir E. Blinov}
\author[22]{Johannes Bloms}
\author[23]{Gianluigi Boca}
\author[19]{Simon Bodenschatz}
\author[5]{Niels Boelger}
\author[24]{Merlin Böhm}
\author[13]{Ralph Böhm}
\author[5]{Stephan Bökelmann}
\author[4]{Michael Bölting}
\author[22]{Daniel Bonaventura}
\author[17]{Alexander Boukharov}
\author[25]{Gianangelo Bracco}
\author[26]{Mario Bragadireanu}
\author[22]{Philipp Brand}
\author[19]{Kai-Thomas Brinkmann}
\author[19]{Lisa Brück}
\author[17]{Marina Bukharova}
\author[2]{Sofia Bukreeva}
\author[27]{Denchay Bumrungkoh}
\author[28,29]{Maria Pia Bussa}
\author[6]{Hans Calen}
\author[29]{Daniela Calvo}
\author[4]{Luigi Capozza}
\author[30]{Michele Caselle}
\author[31]{Bo Cederwall}
\author[32]{Vinee Chauhan}
\author[16]{Viacheslav Chernetsky}
\author[30]{Suren Chilingaryan}
\author[5]{Sebastian Coen}
\author[3]{Oliver Corell}
\author[33]{Volker Crede}
\author[18]{Fabrizio Davì}
\author[5]{Remco de Boer}
\author[29]{Paolo De Remigis}
\author[16]{Alexey Demekhin}
\author[3]{Achim Denig}
\author[34]{Haluk Denizli}
\author[7]{Harald Deppe}
\author[9]{Artur Derichs}
\author[19]{Stefan Diehl}
\author[19]{Lara Dippel}
\author[33]{Sean Dobbs}
\author[1]{Valery Kh. Dodokhov}
\author[16]{Anatoly Dolgolenko}
\author[35]{Mariusz Domagala}
\author[12]{Maria Doncel Monasterio}
\author[19]{Valery Dormenev}
\author[9]{Rene Dosdall}
\author[30]{Timo Dritschler}
\author[36]{Daniel Duda}
\author[19]{Michael Düren}
\author[7]{Roman Dzhygadlo}
\author[1]{Alexander Efremov}
\author[22]{Hanna Eick}
\author[34]{Nuray Er}
\author[19]{Thorsten Erlen}
\author[11]{Alexandr Erokhin}
\author[7]{Waleed Esmail}
\author[33]{Paul Eugenio}
\author[24]{Wolfgang Eyrich}
\author[19]{Aniko Falk}
\author[16]{Pavel Fedorets}
\author[37]{Gleb Fedotov}
\author[5]{Florian Feldbauer}
\author[2]{Valeri Ferapontov}
\author[29]{Alessandra Filippi}
\author[35]{Grzegorz Filo}
\author[38]{Michael Finger, Jr.}
\author[38]{Miroslav Finger}
\author[5]{Mario Fink}
\author[39]{Miroslaw Firlej}
\author[39]{Tomasz Fiutowski}
\author[7]{Holger Flemming}
\author[5]{Jens Frech}
\author[32]{Celina Marie Frenkel}
\author[5]{Miriam Fritsch}
\author[1]{Aida Galoyan}
\author[40]{Keval Gandhi}
\author[16]{Alexander Gerasimov}
\author[7]{Andreas Gerhardt}
\author[19]{Kim Tabea Giebenhain}
\author[7]{Daniel Glaab}
\author[41]{Derek Glazier}
\author[19]{Simon Glennemeier-Marke}
\author[9]{Frank Goldenbaum}
\author[1]{Georgy Golovanov}
\author[16]{Alexander Golubev}
\author[2]{Yury Goncharenko}
\author[7]{Klaus Götzen}
\author[4]{Boxing Gou}
\author[24]{Katja Gumbert}
\author[5]{Rene Hagdorn}
\author[19]{Christopher Hahn}
\author[32]{Christian Hammann}
\author[32]{Jan Hartmann}
\author[30]{Greta Heine}
\author[5]{Fritz-Herbert Heinsius}
\author[7]{Andreas Heinz}
\author[5]{Thomas Held}
\author[42]{Christoph Herold}
\author[22]{Benjamin Hetz}
\author[43]{Mathilde Himmelreich}
\author[3]{Matthias Hoek}
\author[19]{Jan Hofmann}
\author[5]{Tobias Holtmann}
\author[5]{Fabian Hölzken}
\author[44]{Guang Shun Huang}
\author[39]{Marek Idzik}
\author[41]{David Ireland}
\author[45]{Vladimir Jary}
\author[43]{Peiyong Jiang}
\author[46]{Zhu Jiang}
\author[6]{Tord Johansson}
\author[47]{Kushal Kalita}
\author[2]{Nikita Kalugin}
\author[9]{Jakapat Kannika}
\author[16]{Alexey Kantsyrev}
\author[7]{Radoslaw Karabowicz}
\author[48]{Alexander Käser}
\author[49]{Dzmitry Kazlou}
\author[19]{Sophie Kegel}
\author[5]{Iman Keshk}
\author[50]{Grazina Kesik}
\author[34]{Umut Keskin}
\author[32]{Bernhard Ketzer}
\author[19]{Faiza Khalid}
\author[22]{Alfons Khoukaz}
\author[5]{Roman Klasen}
\author[5,7]{Ralf Kliemt}
\author[42]{Chinorat Kobdaj}
\author[5]{Helmut Koch}
\author[7]{Stefan Koch}
\author[32]{Jonas Kohlen}
\author[21]{Sergey Kononov}
\author[5]{Bertram Kopf}
\author[30]{Andreas Kopmann}
\author[45]{Oleksandr Korchak}
\author[51]{Grzegorz Korcyl}
\author[52]{Krzysztof Korcyl}
\author[49]{Mikhail Korzhik}
\author[50]{Tymoteusz Kosinski}
\author[50]{Natalia Kozak}
\author[24]{Steffen Krauss}
\author[21]{Evgeniy A. Kravchenko}
\author[19]{Aron Kripko}
\author[16]{Nikolai Kristi}
\author[53]{Marcel Kunze}
\author[6]{Andrzej Kupsc}
\author[7]{Udo Kurilla}
\author[5]{Meike Küßner}
\author[1]{Sergey Kutuzov}
\author[11]{Ivan A. Kuyanov}
\author[38]{Antonin Kveton}
\author[16]{Elena Ladygina}
\author[51]{Rafal Lalik}
\author[18]{Giovanni Lancioni}
\author[54]{Mark Lattery}
\author[3]{Werner Lauth}
\author[52]{Piotr Lebiedowicz}
\author[24]{Albert Lehmann}
\author[7]{Dorothee Lehmann}
\author[13,41]{Inti Lehmann}
\author[3]{Hans Heinrich Leithoff}
\author[2]{Andrei Levin}
\author[5]{Jinxin Li}
\author[55]{Yutie Liang}
\author[42]{Ayut Limphirat}
\author[5]{Lukas Linzen}
\author[35]{Edward Lisowski}
\author[56]{Beijiang Liu}
\author[56]{Chunxiu Liu}
\author[44]{Dong Liu}
\author[56]{Zhenan Liu}
\author[57]{Herbert Loehner}
\author[58]{Vincenzo Lucherini}
\author[7]{Jost Lühning}
\author[16]{Elena Luschevskaya}
\author[7]{Uli Lynen}
\author[4]{Frank Maas}
\author[5]{Stephan Maldaner}
\author[51]{Akshay Malige}
\author[17]{Oleg Malyshev}
\author[37]{Sergey Manaenkov}
\author[27]{Keerati Manasatitpong}
\author[22]{Christian Mannweiler}
\author[6]{Pawel Marciniewski}
\author[45]{Michal Marcisovsky}
\author[10]{Johann Marton}
\author[2]{Eseniya Maslova}
\author[50]{Michal Matusiak}
\author[16]{Vladimir A. Matveev}
\author[29]{Giovanni Mazza}
\author[50]{Dmytro Melnychuk}
\author[18]{Paolo Mengucci}
\author[3]{Harald Merkel}
\author[7]{Johan Messchendorp}
\author[35]{Mateusz Michałek}
\author[24]{Daniel Miehling}
\author[37]{Oleg Miklukho}
\author[2]{Nikolay Minaev}
\author[49]{Oleg Missevitch}
\author[2,17]{Vasiliy V. Mochalov}
\author[2]{Vyacheslav Moiseev}
\author[39]{Aleksandra Molenda}
\author[18]{Luigi Montalto}
\author[39]{Jakub Moron}
\author[2]{Dmitry Morozov}
\author[4]{Christof Motzko}
\author[3]{Ulrich Müller}
\author[32]{Johannes Müllers}
\author[42]{Thanachot Nasawad}
\author[18]{Pier Paolo Natali}
\author[7]{Frank Nerling}
\author[2]{Larisa Nogach}
\author[4]{Oliver Noll}
\author[2]{Konstantin Novikov}
\author[45]{Josef Novy}
\author[51]{Krzysztof Nowakowski}
\author[59]{Asiye Tugba Olgun}
\author[9]{Sergey Orfanitski}
\author[19]{Pavel Orsich}
\author[4]{Herbert Orth}
\author[16]{Vsevolod Panjushkin}
\author[5]{Sven Pankonin}
\author[16]{Alena Panyuschkina}
\author[18]{Nicola Paone}
\author[6]{Michael Papenbrock}
\author[5]{Marc Pelizäus}
\author[44]{Hai Ping Peng}
\author[9]{Gabriela Perez-Andrade}
\author[19]{Marvin Peter}
\author[7]{Klaus Peters}
\author[3,4]{Jannik Petersen}
\author[1]{Alexey A. Piskun}
\author[11]{Sergey Pivovarov}
\author[3]{Josef Pochodzalla}
\author[27]{Surachai Pongampai}
\author[35]{Piotr Poznanski}
\author[9]{Dieter Prasuhn}
\author[38]{Ivan Prochazka}
\author[51]{Witold Przygoda}
\author[11]{Evgeniy Pyata}
\author[52]{Krzysztof Pysz}
\author[35]{Joanna Płazek}
\author[44]{Hang Qi}
\author[60]{Jiajia Quin}
\author[40]{Ajay Kumar Rai}
\author[51]{Narendra Rathod}
\author[19]{Andreas Reeh}
\author[7]{Jenny Regina}
\author[5]{Jan Reher}
\author[5]{Gerhard Reicherz}
\author[6]{Jana Rieger}
\author[61]{Valentino Rigato}
\author[18]{Daniele Rinaldi}
\author[7,9,5]{James Ritman}
\author[7]{Elena Rocco}
\author[4]{David Rodríguez Piñeiro}
\author[4]{Christoph Rosner}
\author[2]{Andrey Ryazantsev}
\author[2]{Sergey Ryzhikov}
\author[19]{Matthias Sachs}
\author[32]{Ben Salisbury}
\author[1]{Alexander Samartsev}
\author[18]{Lorenzo Scalise}
\author[7]{Susan Schadmand}
\author[52]{Wolfgang Schäfer}
\author[7]{Georg Schepers}
\author[3]{Soeren Schlimme}
\author[7]{Christian Joachim Schmidt}
\author[32]{Christoph Schmidt}
\author[19]{Mustafa Schmidt}
\author[13]{Lars Schmitt}
\author[5]{Claudius Schnier}
\author[6]{Karin Schönning\fnref{label2}}
\author[19]{René Schubert}
\author[4]{Falk Schupp}
\author[7]{Carsten Schwarz}
\author[7]{Joachim Schwiening}
\author[9]{Thomas Sefzick}
\author[32]{Tobias Seifen}
\author[41]{Bjoern Seitz}
\author[2,17]{Pavel A. Semenov}
\author[62]{Kam Seth}
\author[3]{Concettina Sfienti}
\author[2]{Igor Shein}
\author[56]{Xiaoyan Shen}
\author[1]{Stepan Shimanski}
\author[42]{Tawanchat Simantathammakul}
\author[1]{Anna N. Skachkova}
\author[38]{Miloslav Slunecka}
\author[51]{Jerzy Smyrski}
\author[5]{Mark Snoeyink}
\author[51]{Bartosz Sobol}
\author[28,29]{Stefano Spataro}
\author[16]{Alexey Valentinovich Stavinskiy}
\author[48]{Michael Steinacher}
\author[4]{Marcell Steinen}
\author[37]{Vladimir Stepanov}
\author[9]{Tobias Stockmanns}
\author[19]{Marcel Straube}
\author[19]{Marc Strickert}
\author[1]{Evgeny A. Strokovsky}
\author[56]{Shengsen Sun}
\author[44]{Yan Kun Sun}
\author[5,7]{Ken Suzuki}
\author[39]{Krzysztof Swientek}
\author[52]{Antoni Szczurek}
\author[19]{Chris N. Takatsch}
\author[50]{Jerzy Tarasiuk}
\author[7]{Alexander Täschner}
\author[59]{Zeynep Tavukoglu}
\author[12]{Per-Erik Tegner}
\author[39]{Przemyslaw Terlecki}
\author[32]{Ulrike Thoma}
\author[11]{Yury Tikhonov}
\author[1]{Valery Tokmenin}
\author[45]{Lukas Tomasek}
\author[63]{Egle Tomasi-Gustafsson}
\author[7]{Michael Traxler}
\author[5]{Tobias Triffterer}
\author[19]{Nils Tröll}
\author[1]{Vladimir Uzhinsky}
\author[13]{Victor Varentsov}
\author[2,17]{Alexander N. Vasiliev}
\author[37]{Denis Veretennikov}
\author[1]{Alexander Verkheev}
\author[22]{Sophia Vestrick}
\author[45]{Miroslav Virius}
\author[17]{Evgeny Vishnevsky}
\author[1]{Alexander Vodopianov}
\author[38]{Michal Volf}
\author[7]{Bernd Voss}
\author[60]{Fei Wang}
\author[19]{Thomas Wasem}
\author[64]{Daniel Watts}
\author[22]{Frederik Weidner}
\author[19]{Leonard Welde}
\author[19]{Katharina Wendlandt}
\author[5]{Christopher Wenzel}
\author[19]{Vincent Wettig}
\author[7]{Peter Wieczorek}
\author[5]{Ulrich Wiedner}
\author[9]{Peter Wintz}
\author[43]{Yannic Wolf}
\author[4]{Sahra Wolff}
\author[6]{Magnus Wolke}
\author[27]{Narupon Wongprachanukul}
\author[50]{Slawomir Wronka}
\author[62]{Ting Xiao}
\author[9]{Huagen Xu}
\author[2]{Alexander Yakutin}
\author[34]{Seda Yerlikaya}
\author[34,65]{Ali Yilmaz}
\author[46]{Chunxu Yu}
\author[50]{Tomasz Zakrzewski}
\author[19]{Hans-Georg Zaunick}
\author[46]{Xiao Zhang}
\author[56]{Guang Zhao}
\author[56]{Jingzhou Zhao}
\author[37]{Andrey Zhdanov}
\author[60]{Bo Zheng}
\author[44]{Xiao Rong Zhou}
\author[46]{Wenjing Zhu}
\author[1]{Nikolai I. Zhuravlev}
\author[4]{Iris Zimmermann}
\author[46]{Zhang Ziyu}
\author[50]{Boguslaw Zwieglinski}
\affiliation[1]{organization={Joint Institute for Nuclear Research},
city={Dubna},
country={Russia}}
\affiliation[2]{organization={A.A. Logunov Institute for High Energy Physics of the National Research Centre “Kurchatov Institute”},
city={Protvino},
country={Russia}}
\affiliation[3]{organization={Johannes Gutenberg-Universität Institut für Kernphysik},
city={Mainz},
country={Germany}}
\affiliation[4]{organization={Helmholtz-Institut Mainz},
city={Mainz},
country={Germany}}
\affiliation[5]{organization={Ruhr-Universität Bochum Institut für Experimentalphysik I},
city={Bochum},
country={Germany}}
\affiliation[6]{organization={Uppsala Universitet Institutionen för fysik och astronomi},
city={Uppsala},
country={Sweden}}
\affiliation[7]{organization={GSI Helmholtzzentrum für Schwerionenforschung GmbH},
city={Darmstadt},
country={Germany}}
\affiliation[8]{organization={European Organization for Nuclear Research (CERN)},
city={Geneva},
country={Switzerland}}
\affiliation[9]{organization={Forschungszentrum Jülich Institut für Kernphysik},
city={Jülich},
country={Germany}}
\affiliation[10]{organization={Stefan Meyer Institute},
city={Wien},
country={Austria}}
\affiliation[11]{organization={Budker Institute of Nuclear Physics},
city={Novosibirsk},
country={Russia}}
\affiliation[12]{organization={Stockholms Universitet},
city={Stockholm},
country={Sweden}}
\affiliation[13]{organization={FAIR Facility for Antiproton and Ion Research in Europe},
city={Darmstadt},
country={Germany}}
\affiliation[14]{organization={Department of Physics Dogus University},
city={Istanbul},
country={Turkey}}
\affiliation[15]{organization={University of Tehran},
city={Tehran},
country={Iran}}
\affiliation[16]{organization={Institute for Theoretical and Experimental Physics named by A.I. Alikhanov of National Research Centre "Kurchatov Institute”},
city={Moscow},
country={Russia}}
\affiliation[17]{organization={Moscow Power Engineering Institute},
city={Moscow},
country={Russia}}
\affiliation[18]{organization={Università Politecnica delle Marche-Ancona},
city={Ancona},
country={Italy}}
\affiliation[19]{organization={Justus-Liebig-Universität Gießen II. Physikalisches Institut},
city={Gießen},
country={Germany}}
\affiliation[20]{organization={Università di Brescia},
city={Brescia},
country={Italy}}
\affiliation[21]{organization={Novosibirsk State University},
city={Novosibirsk},
country={Russia}}
\affiliation[22]{organization={Westfälische Wilhelms-Universität Münster},
city={Münster},
country={Germany}}
\affiliation[23]{organization={Dipartimento di Fisica Università di Pavia INFN Sezione di Pavia},
city={Pavia},
country={Italy}}
\affiliation[24]{organization={Friedrich-Alexander-Universität Erlangen-Nürnberg},
city={Erlangen},
country={Germany}}
\affiliation[25]{organization={Dept of Physics University of Genova and INFN-Genova},
city={Genova},
country={Italy}}
\affiliation[26]{organization={Institutul National de C\&D pentru Fizica si Inginerie Nucleara "Horia Hulubei"},
city={Bukarest-Magurele},
country={Romania}}
\affiliation[27]{organization={Synchrotron Light Research Institute},
city={Nakhon Ratchasima},
country={Thailand}}
\affiliation[28]{organization={Università di Torino and INFN Sezione di Torino},
city={Torino},
country={Italy}}
\affiliation[29]{organization={INFN Sezione di Torino},
city={Torino},
country={Italy}}
\affiliation[30]{organization={Karlsruhe Institute of Technology Institute for Data Processing and Electronics},
city={Karlsruhe},
country={Germany}}
\affiliation[31]{organization={Kungliga Tekniska Högskolan},
city={Stockholm},
country={Sweden}}
\affiliation[32]{organization={Rheinische Friedrich-Wilhelms-Universität Bonn},
city={Bonn},
country={Germany}}
\affiliation[33]{organization={Florida State University},
city={Tallahassee},
country={U.S.A.}}
\affiliation[34]{organization={Bolu Abant Izzet Baysal University},
city={Bolu},
country={Turkey}}
\affiliation[35]{organization={University of Technology Institute of Applied Informatics},
city={Cracow},
country={Poland}}
\affiliation[36]{organization={University of West Bohemia},
city={Pilsen},
country={Czech Republic}}
\affiliation[37]{organization={National Research Centre "Kurchatov Institute" B. P. Konstantinov Petersburg Nuclear Physics Institute Gatchina},
city={St. Petersburg},
country={Russia}}
\affiliation[38]{organization={Charles University Faculty of Mathematics and Physics},
city={Prague},
country={Czech Republic}}
\affiliation[39]{organization={AGH University of Science and Technology},
city={Cracow},
country={Poland}}
\affiliation[40]{organization={Sardar Vallabhbhai National Institute of Technology Applied Physics Department},
city={Surat},
country={India}}
\affiliation[41]{organization={University of Glasgow},
city={Glasgow},
country={United Kingdom}}
\affiliation[42]{organization={Suranaree University of Technology},
city={Nakhon Ratchasima},
country={Thailand}}
\affiliation[43]{organization={Goethe-Universität},
city={Institut für Kernphysik},
country={Frankfurt}}
\affiliation[44]{organization={University of Science and Technology of China},
city={Hefei},
country={China}}
\affiliation[45]{organization={Czech Technical University Faculty of Nuclear Sciences and Physical Engineering},
city={Prague},
country={Czech Republic}}
\affiliation[46]{organization={Nankai University},
city={Nankai},
country={China}}
\affiliation[47]{organization={Gauhati University Physics Department},
city={Guwahati},
country={India}}
\affiliation[48]{organization={Universität Basel},
city={Basel},
country={Switzerland}}
\affiliation[49]{organization={Research Institute for Nuclear Problems Belarus State University},
city={Minsk},
country={Belarus}}
\affiliation[50]{organization={National Centre for Nuclear Research},
city={Warsaw},
country={Poland}}
\affiliation[51]{organization={Instytut Fizyki Uniwersytet Jagiellonski},
city={Cracow},
country={Poland}}
\affiliation[52]{organization={IFJ Institute of Nuclear Physics PAN},
city={Cracow},
country={Poland}}
\affiliation[53]{organization={Universität Heidelberg},
city={Heidelberg},
country={Germany}}
\affiliation[54]{organization={University of Wisconsin Oshkosh},
city={Oshkosh},
country={U.S.A.}}
\affiliation[55]{organization={Chinese Academy of Science Institute of Modern Physics},
city={Lanzhou},
country={China}}
\affiliation[56]{organization={Institute of High Energy Physics Chinese Academy of Sciences},
city={Beijing},
country={China}}
\affiliation[57]{organization={Energy and Sustainability Research Institute (ESRIG) University of Groningen},
city={Groningen},
country={Netherlands}}
\affiliation[58]{organization={INFN Laboratori Nazionali di Frascati},
city={Frascati},
country={Italy}}
\affiliation[59]{organization={Istanbul Okan University},
city={Istanbul},
country={Turkey}}
\affiliation[60]{organization={University of South China},
city={Hengyang},
country={China}}
\affiliation[61]{organization={INFN Laboratori Nazionali di Legnaro},
city={Legnaro},
country={Italy}}
\affiliation[62]{organization={Northwestern University},
city={Evanston},
country={U.S.A.}}
\affiliation[63]{organization={IRFU CEA Université Paris-Saclay},
city={Gif-sur-Yvette Cedex},
country={France}}
\affiliation[64]{organization={University of Edinburgh},
city={Edinburgh},
country={United Kingdom}}
\affiliation[65]{organization={Giresun University},
city={Giresun},
country={Turkey}}


